Extract Dynamic Information To Improve Time Series Modeling: a Case Study with Scientific Workflow

In modeling time series data, we often need to augment the existing data records to increase the modeling accuracy. In this work, we describe a number of techniques to extract dynamic information about the current state of a large scientific workflow, which could be generalized to other types of applications. The specific task to be modeled is the time needed for transferring a file from an experimental facility to a data center. The key idea of our approach is to find recent past data transfer events that match the current event in some ways. Tests showed that we could identify recent events matching some recorded properties and reduce the prediction error by about 12% compared to the similar models with only static features. We additionally explored an application specific technique to extract information about the data production process, and was able to reduce the average prediction error by 44%.

==> Makefile <==
###############################################################################
# the latex command is pdflatex
LATEX = pdflatex

###############################################################################
# the main latex file is jfds2019.tex in this directory
MAIN = main

###############################################################################
# Assume all LaTeX files (*.tex) are in this level and all figures are in figs
# directory and all bibtex entries are at this level with .bib
TEXFILES = ${wildcard *.tex} ${wildcard neural_net/*.tex} ${wildcard ANA/*.tex} ${wildcard FFB/*.tex} ${wildcard *.cls} ${wildcard *.clo} ${wildcard *.sty}
BIBFILES = ${wildcard *.bib} ${wildcard neural_net/*.bib}
FIGS = ${wildcard figures/*.png} ${wildcard figures/*.pdf} ${wildcard figures/*.jpg} ${wildcard neural_net/figures/*.png} ${wildcard neural_net/figures/*.pdf} ${wildcard neural_net/figures/*.jpg}

###############################################################################
# default target
.DEFAULT_GOAL := $(MAIN).pdf
$(MAIN): $(MAIN).pdf
.PHONY: $(MAIN) clean realclean

###############################################################################
# run LATEX command to generate the main PDF file
$(MAIN).pdf $(MAIN).log: $(TEXFILES) $(FIGS) $(BIBFILES)
	${LATEX} $(MAIN)
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	bibtex $(MAIN); ${LATEX} $(MAIN); fi;
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	bibtex $(MAIN); ${LATEX} $(MAIN); fi;
	@while grep 'Rerun to get ' $(MAIN).log; \
        do ${LATEX} $(MAIN); \
        done

draft1.pdf draft1.log: $(TEXFILES) $(FIGS) $(BIBFILES)
	${LATEX} draft1
	@if [ `fgrep undefined draft1.log | fgrep Citation - | wc -l` -gt 0 ]; then \
	bibtex draft1; ${LATEX} draft1; fi;
	@if [ `fgrep undefined draft1.log | fgrep Citation - | wc -l` -gt 0 ]; then \
	bibtex draft1; ${LATEX} draft1; fi;
	@while grep 'Rerun to get ' draft1.log; \
        do ${LATEX} draft1; \
        done

###############################################################################
# basic sanity check
check: missingincludes badrefs badbibs

# Extract a list of missing smartinclude files
missingincludes: $(MAIN).log
	@(grep -i "smartinclude: warning:" $< | \
	  sed 's/smartinclude: WARNING: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== SMARTINCLUDE WARNINGS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check log for: 
# - Multiply defined labels
# - Undefined labels
# - Undefined citations
# - Undefined acronyms (no messages for multiply-defined acronyms)
badrefs: $(MAIN).log
	@(grep -i "latex warning:" $< |\
	  grep -v -i "there were multiply-defined labels" | \
	  grep "multiply defined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MULTIPLY-DEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "latex warning:" $< | \
	  grep -v -i "there were undefined references" | \
	  grep -i "reference" | grep -i "undefined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "package acronym warning:" $< | \
	  grep -i "acronym" | grep -i "not defined" |\
	  sed 's/Package acronym Warning: //' |\
	  sort | uniq > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED ACRONYMS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check BibTeX log for:
# - missing .bib files
# - missing database entries
# - repeated entries
# - string name undefined
# - errors in entries ("I was expecting...")
badbibs: $(MAIN).log
	bibtex $(MAIN)
	@(grep -i "i couldn't open database file " $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB FILES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--i didn't find a database entry for" \
	  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "repeated entry--"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== REPEATED BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--string name" $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED STRINGS IN BIB =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "i was expecting"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== ERRORS IN BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

clean:
	-@find . \( -name '*.aux' -print \) -o \( -name '*.log' -print \) \
		-o \( -name '*.bbl' -print \) -o \( -name '*.blg' -print \) \
		-o \( -name '*.toc' -print \) -o \( -name '*.out' -print \) \
		-o \( -name '*.fff' -print \) -o \( -name '*~' -print \) \
		-o \( -name '*.maf' -print \) -o \( -name '*.mtc*' -print \) | xargs $(RM)

###############################################################################
# WARNING: removes the main target
realclean: clean
	$(RM) $(MAIN).pdf* draft1.pdf*

